APO Time Resolved Color Photometry of Highly-Elongated Interstellar Object 1I/'Oumuamua

We report on $g$, $r$ and $i$ band observations of the Interstellar Object 'Oumuamua (1I) taken on 2017 October 29 from 04:28 to 08:40 UTC by the Apache Point Observatory (APO) 3.5m telescope's ARCTIC camera. We find that 1I's colors are $g-r=0.41\pm0.24$ and $r-i=0.23\pm0.25$, consistent with the visible spectra of Masiero (2017), Ye et al. (2017) and Fitzsimmons et al. (2017), and most comparable to the population of Solar System C/D asteroids, Trojans, or comets. We find no evidence of any cometary activity at a heliocentric distance of 1.46 au, approximately 1.5 months after 1I's closest approach distance to the Sun. Significant brightness variability was seen in the $r$ observations, with the object becoming notably brighter towards the end of the run. By combining our APO photometric time series data with the Discovery Channel Telescope (DCT) data of Knight et al. (2017), taken 20 h later on 2017 October 30, we construct an almost complete light curve with a most probable lightcurve period of $P \simeq 4~{\rm h}$. Our results imply a double peaked rotation period of 8.1 $\pm$ 0.02 h, with a peak-to-peak amplitude of 1.5 - 2.1 mags. Assuming that 1I's shape can be approximated by an ellipsoid, the amplitude constraint implies that 1I has an axial ratio of 3.5 to 10.3, which is strikingly elongated. Assuming that 1I is rotating above its critical break up limit, our results are compatible with 1I having having modest cohesive strength and may have obtained its elongated shape during a tidal disruption event before being ejected from its home system. Astrometry useful for constraining 1I's orbit was also obtained and published in Weaver et al. (2017).

==> newcommands.tex <==

% Handy macros...


%%Fix same author same year references
\newcommand{\sameyear}[1]{}

%footnote
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

% latex short form notation
\newcommand{\tnm}[1]{{\tablenotemark{#1}}}
\newcommand{\tnt}[2]{{\tablenotetext{#1}{#2}}}

%abbreviations
\newcommand{\eg}{{\it e.g.}}
\newcommand{\Eg}{{\it E.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
\newcommand{\etal}{{\it et~al.}}
\newcommand{\adhoc}{{\it ad~hoc}}
\newcommand{\apriori}{{\it a~priori}}
\newcommand{\postfacto}{{\it post~facto}}


%math
\newcommand{\half}{{1\over2}}
\newcommand{\mean}[1]{\langle{#1}\rangle}
\newcommand{\dif}{\mathrm{d}}
\newcommand{\iint}[2]{\int\!\!\!\int\limits_{#1}^{#2}}
\newcommand{\iiint}[2]{\int\!\!\!\int\limits_{#1}^{#2}\!\!\!\int}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\oforder}{\mathcal{O}}
\newcommand{\logten}{\mathrm{\log_{10}}}

%orbits
\newcommand{\xyz}{(x,y,z)}
\newcommand{\xyzdot}{(\dot{x},\dot{y},\dot{z})}
\newcommand{\aei}{(a,e,i)}
\newcommand{\aeiH}{(a,e,i,H)}
\newcommand{\OoM}{(\Omega,\omega,M)}
\newcommand{\vo}{\vec{o}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vxdot}{\vec{\dot x}}
\newcommand{\vxavg}{\mean{\vec{x}}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vyavg}{\mean{\vec{y}}}
\newcommand{\vz}{\vec{z}}
\newcommand{\vzavg}{\mean{\vec{z}}}
\newcommand{\Havg}{\mean{H}}
\newcommand{\ep}{\mathrm{e_p}}
\newcommand{\ip}{\mathrm{i_p}}

%variables
\newcommand{\x}{ \; \mathrm{x} \;}

%editing
\newcommand{\todo}[2]{{\bf #1 - #2}}
\newcommand{\note}[2]{{{\bf #1} - {\it #2}}}
\newcommand{\XXX}{{\bf XXX}}
\newcommand{\bb}[1]{{{\bf BB : \bf #1}}}

%miscellaneous
\newcommand{\sn}{$S/N$}
\newcommand{\SN}{$S/N$}
%\newcommand{\th}{$^{th}$}  % already defined somewhere else?
\newcommand{\rd}{$^{rd}$}
\newcommand{\st}{$^{st}$}
\newcommand{\nd}{$^{nd}$}

%units
%\newcommand{\arcmin}{^{\prime}}
%\newcommand{\arcsec}{^{\prime\prime}}
\newcommand{\h}{^\mathrm{h}}
\newcommand{\m}{^\mathrm{m}}
\newcommand{\mic}{\mathrm{\mu m}}
\newcommand{\s}{^\mathrm{s}}
\newcommand{\Mpc}{\,\mathrm{Mpc}}
\newcommand{\kpc}{\,\mathrm{kpc}}
%\newcommand{\mps}{\,\mathrm{m \; s^{-1}}}
\newcommand{\mps}{\,\mathrm{m\;s^{-1}}}
%\newcommand{\kmps}{\,\mathrm{km \; s^{-1}}}
\newcommand{\kmps}{\,\mathrm{\frac{km}{s}}}
\newcommand{\gpcmc}{\,\mathrm{g \; cm^{-3}}}
\newcommand{\pc}{\,\mathrm{pc}}
\newcommand{\au}{\,\mathrm{au}}
\newcommand{\km}{\,\mathrm{km}}
\newcommand{\kph}{\,\mathrm{km}/\mathrm{h}}
\newcommand{\ft}{\,\mathrm{ft}}
\newcommand{\meter}{\,\mathrm{m}}
\newcommand{\cm}{\,\mathrm{cm}}
\newcommand{\mm}{\,\mathrm{mm}}
\newcommand{\um}{\,\mu \mathrm{m}}
\newcommand{\nm}{\,\mathrm{nm}}
\newcommand{\rad}{\,\mathrm{rad}}
\newcommand{\anno}{\,\mathrm{a}}
\newcommand{\yr}{\,\mathrm{yr}}
\newcommand{\days}{\,\mathrm{d}}
\newcommand{\myr}{\,\mathrm{Myr}}
\newcommand{\gyr}{\,\mathrm{Gyr}}
\newcommand{\vrk}{\,\mathrm{vrk}}
\newcommand{\degrees}{\,\mathrm{deg}}
\newcommand{\hours}{\,hours}
\newcommand{\hour}{\,\mathrm{h}}
\newcommand{\minute}{\,\mathrm{min}}
\newcommand{\second}{\,\mathrm{s}}
\newcommand{\magnitude}{\,\mathrm{mag}}
\newcommand{\K}{\,\mathrm{K}}
\newcommand{\J}{\,\mathrm{J}}
\newcommand{\N}{\,\mathrm{N}}
\newcommand{\kg}{\,\mathrm{kg}}
\newcommand{\g}{\,\mathrm{g}}
\newcommand{\z}{\,\mathrm{z}}
\newcommand{\AMU}{\,\mathrm{AMU}}
\newcommand{\W}{\,\mathrm{W}}
\newcommand{\MW}{\,\mathrm{MW}}
\newcommand{\degC}{\arcdeg\mathrm{C}}
\newcommand{\degK}{\arcdeg\mathrm{K}}
\newcommand{\pv}{p_V}
\newcommand{\pir}{\mathrm{p_IR}}
\newcommand{\gcmv}{\mathrm{g \; cm^{-3}}}
\newcommand{\conductivity}{\mathrm{W \; m^{-1} \; K^{-1}}}
\newcommand{\tdeg}{^{\circ}}
\newcommand{\invyr}{\mathrm{yr^{-1}}}
\newcommand{\invau}{\mathrm{au^{-1}}}
\newcommand{\invkm}{\mathrm{km^{-1}}}
%\newcommand{\sin}{\mathrm{sin}}


%asteroids
\newcommand{\TC}{{2008~TC$_3$}}
\newcommand{\RH}{{2006~RH$_{120}$}}
\newcommand{\FY}{{1993~FY$_{12}\;$}}
\newcommand{\FYnospace}{{1993~FY$_{12}$}}
%\newcommand{\1I}{{1I/`Oumuamua}}
\newcommand{\oumTITLE}{{1I/`OUMUAMUA}}
\newcommand{\oum}{{1I/`Oumuamua}}
\newcommand{\oumspace}{{1I/`Oumuamua }}
% from
% PS-1 Latex template v. 7.0 C. Stubbs June 14 2011 (with thanks to Tex-gurus Michael Wood-Vasey, Gautham Narayan, and Ryan Foley)

%filters
\newcommand{\gps}{\ensuremath{g_{\rm P1}}}
\newcommand{\rps}{\ensuremath{r_{\rm P1}}}
\newcommand{\ips}{\ensuremath{i_{\rm P1}}}
\newcommand{\zps}{\ensuremath{z_{\rm P1}}}
\newcommand{\yps}{\ensuremath{y_{\rm P1}}}
\newcommand{\wps}{\ensuremath{w_{\rm P1}}}
\newcommand{\grizy}{\gps\rps\ips\zps\yps}
\newcommand{\JHK}{\ensuremath{JHK}}
\newcommand{\V}{\ensuremath{V}}

% Pan-STARRS
\newcommand{\PS}{\protect \hbox {Pan-STARRS}}
\newcommand{\PSone}{\protect \hbox {Pan-STARRS1}}
\newcommand{\PStwo}{\protect \hbox {Pan-STARRS2}}
\newcommand{\PSfour}{\protect \hbox {Pan-STARRS4}}
\newcommand{\knownserver}{{\tt known\_server}}


